Non-blind watermarking of network flows

Linking network flows is an important problem in intrusion detection as well as anonymity. Passive traffic analysis can link flows but requires long periods of observation to reduce errors. Active traffic analysis, also known as flow watermarking, allows for better precision and is more scalable. Previous flow watermarks introduce significant delays to the traffic flow as a side effect of using a blind detection scheme; this enables attacks that detect and remove the watermark, while at the same time slowing down legitimate traffic. We propose the first non-blind approach for flow watermarking, called RAINBOW, that improves watermark invisibility by inserting delays hundreds of times smaller than previous blind watermarks, hence reduces the watermark interference on network flows. We derive and analyze the optimum detectors for RAINBOW as well as the passive traffic analysis under different traffic models by using hypothesis testing. Comparing the detection performance of RAINBOW and the passive approach we observe that both RAINBOW and passive traffic analysis perform similarly good in the case of uncorrelated traffic, however, the RAINBOW detector drastically outperforms the optimum passive detector in the case of correlated network flows. This justifies the use of non-blind watermarks over passive traffic analysis even though both approaches have similar scalability constraints. We confirm our analysis by simulating the detectors and testing them against large traces of real network flows.

==> background.tex <==
\section{Background}
\label{sec:background}

In this section, we review the problem of detecting stepping stones and then review both the passive and active
approaches to the problem.  We compare the advantages and disadvantages of the two techniques, 
motivating our approach.

% XXX Threat model

\subsection{Stepping Stone Detection}

A stepping stone is a host that is used to relay traffic through an enterprise network to another remote destination.
Stepping stones are used to disguise the true origin of an attack.  Detecting stepping stones can help trace 
attacks back
to their true source.  Also, stepping stones are often indicative of a compromised machine.  
Thus detecting stepping stones is a useful part of enterprise security monitoring.



% \begin{figure*}[!t]
% 	\subfigure[A stepping stone]{
% 		\includegraphics[width=0.48\textwidth]{Figures/stepping-stone}
% 		\label{fig:stepstone}
% 	}
% 	\subfigure[Network flow watermarks]{
% 		\includegraphics[width=0.48\textwidth]{Figures/stepping-stone-wm}
% 		\label{fig:watermark}
% 	}
% 	\caption{Stepping Stone Detection}
% \end{figure*}

Generally, stepping stones are detected by noticing that an outgoing
flow from an enterprise matches an incoming flow.   
%For example, in Figure~\ref{fig:stepstone}, flow 2 will have the same characteristics as flow 5.  
Since the relayed connections are often encrypted (using SSH~\cite{ssh:rfc4251}, for
example), only characteristics such as packet sizes, counts, and
timings are available for such detection. And even these are not
perfectly replicated from an incoming flow to an outgoing flow, as
they are changed by padding schemes, retransmissions, and jitter.
As a result, statistical methods are used to detect correlations
among the incoming and outgoing flows. We next review the passive
and active approaches.

\subsection{Passive Traffic Analysis}

In general, passive traffic analysis techniques operate by recording characteristics of incoming streams 
and then correlating them with outgoing ones.  The right place to do this is often at the border router 
of an enterprise, so the overhead of this technique is the space used to store the stream characteristics 
long enough to check against correlated relayed streams, and the CPU time needed to perform the correlations.  
In a complex enterprise with many interconnected networks, a connection relayed through a stepping stone may 
enter and leave the enterprise through different points; in such cases, there is additional communications 
overhead for transmitting traffic statistics between border routers.

The passive schemes have explored using various characteristics for correlating streams.  Zhang and 
Paxson~\cite{zhang:sec00} model interactive flows as on--off processes and detect linked flows by 
matching up their on--off behavior.  Wang et al.~\cite{wang:esorics02} focus on inter-packet delays, and consider 
several different metrics for correlation.  More recently,
He and Tong used packet counts for stepping stone detection~\cite{he:tosp07}.

Donoho et al. were the first to consider intruder evasion techniques~\cite{donoho:raid02}.  They defined 
a \emph{maximum-tolerable-delay} (MTD) model of attacker evasion and suggested wavelet methods to detect stepping 
stones while being robust to adversarial action.  Blum et al. used a Poisson model of flows to create a technique 
with provable upper bounds on false positive rates~\cite{blum:raid04}, given the MTD model.  However, for 
realistic settings, their techniques require thousands of packets to be observed to achieve reasonable 
rates of false errors.

\subsection{Watermarks}

To address some of the efficiency concerns of passive traffic
analysis, Wang et al. proposed the use of
watermarks~\cite{wang:ccs03}.  In this scenario, a border router
will modify the traffic timings of the incoming flows to contain a
particular pattern---the watermark.  If the same pattern is present
in an outgoing flow, a stepping stone is detected.  
%This can be seen in Figure~\ref{fig:watermark}.

Watermarks improve upon passive traffic analysis in two ways.  First, by inserting a pattern that is 
uncorrelated with any other flows, they can improve the detection efficiency, requiring smaller numbers of 
packets to be observed (hundreds instead of thousands) and providing lower false-positive rates 
($10^{-4}$ or lower, as compared to $10^{-2}$ with passive watermarks).  Second, they can operate in a 
\emph{blind} fashion: after an incoming flow is watermarked, there is no need to record or communicate the 
flow characteristics, since the presence of a watermark can be detected independently.  The detection is also 
potentially faster, as here is no need to compare each outgoing flow to all the incoming flows within the same 
time frame.

Watermarking techniques for network flows have been based on existing techniques for multi-media watermarking.  
For example, Wang et al. based their scheme on QIM
watermarks~\cite{chen:vlsisp01}.  Two other watermark schemes~\cite{pyun:infocom07,wang:oakland07} are 
based on patchwork watermarking~\cite{bender:ibmsys96}, and Yu et al.~\cite{yu:oakland07} developed one 
based on spread-spectrum techniques~\cite{cox:toip97}.  Some of the schemes target anonymous communication 
rather than stepping stones as the application area (both involve the problem of linking flows), but 
the techniques for both are comparable.

\subsection{Watermark Properties}

To motivate our design, we first propose some desirable properties of network flow watermarks.  First of all, 
a watermark should be \emph{robust} to modifications of the traffic characteristics that will occur inside an 
enterprise network, such as jitter.  Watermarks should also be resilient to an adversary who actively tries 
to remove them from the flow, a property we call \emph{active robustness}.  The watermarks should also introduce 
little \emph{distortion}, in that they should not significantly impact the performance of the flows.  This 
is important because in a stepping-stone scenario, most watermarked flows will be benign.  Finally,
watermarks should be \emph{invisible} even to attackers who specifically try to test for their presence.

Looking at previous designs, all of them fail to be invisible: the watermarks introduce large delays, on 
the order of hundreds of milliseconds, on some packets, which can be easily detected by an 
attacker~\cite{peng:oakland06}.  In fact, they cannot even be considered low-distortion, as such large delays 
are easily noticeable and bothersome to legitimate users.  The watermarks are also not actively robust, 
as demonstrated by recent attacks~\cite{peng:oakland06,kiyavash:sec08}.

We also observe that active robustness and invisibility are likely
to be impossible to achieve at the same time.  This is because to be
invisible, the watermark can only introduce minute changes to the
packet stream.  In particular, it cannot introduce jitter of more
than a few milliseconds, since otherwise it will be possible to tell
it apart from the natural network jitter.  However, an active attacker will be
willing to introduce large delays to the network; for example, the
maximum tolerable delay suggested in previous work is 500ms.  As
such, he will be able to destroy any low-order effects that will be
introduced by the watermark.

Further, it is easy to imagine an attacker determined to hide his tracks using even more drastic measures, 
such as using dummy packets to generate a completely independent Poisson process~\cite{blum:raid04}, which 
will render any linking techniques ineffective.  As such, we decided to design a watermark scheme that is 
robust to normal network interference, though not actively robust, and is invisible.  This will serve to 
detect stepping stones where attackers are unwilling (or unable) to actively distort their stream as it 
crosses a stepping stone.  Further, as the watermark will be invisible, attackers will not be able to tell 
if they are being traced and thus will be less likely to try to apply costly watermark countermeasures.


==> conclusions.tex <==

\section{Conclusions\label{sec:conclusionsFuturework}}

%We proposed a novel non-blind network flow watermarking scheme called RAINBOW, for linking flows.
%RAINBOW combines some of the advantages of passive traffic analysis with watermarking schemes.
%Like passive traffic analysis, RAINBOW does not interfere with regular users by inserting
%large delays that are used in existing watermarking schemes; in fact, we show that
%RAINBOW is \emph{invisible} to detection by an attacker.  Like other watermarking schemes,
%RAINBOW achieves very low false error rates.  In fact, we show, both through analysis
%and by means of experiment, that the false error rates of RAINBOW are orders of magnitude lower for
%short observation periods than existing passive and active schemes.  RAINBOW can also be made robust
%to high rates of packet addition and removal by introducing selective correlation, at the cost of
%somewhat increased observation period lengths.  In our future work, we intend to explore coding tools to increase the
%efficiency of RAINBOW and explore the possibility of a blind or semi-blind watermark scheme that remains invisible.

In this paper, we introduce the first non-blind active traffic analysis scheme, RAINBOW.
Using the tools from the detection and estimation theory, we find the optimum passive and (non-blind) active traffic analysis schemes for different types of the network flows. 
We show that, for different traffic models,  the optimum active detectors outperform the optimum passive detectors. This advantage is more significant for the more correlated network traffic, e.g., the web browsing traffic. Considering the fact that both passive and non-blind active approaches of traffic analysis are constrained by similar scalability issues, this finding motivated the use of non-blind active approaches over the passive approaches. 


==> introduction.tex <==

 
\section{Introduction}

Internet attackers commonly relay their traffic through a number of 
(usually compromised) hosts in order to hide their identity.  Detecting 
such hosts, called stepping stones, is therefore an important problem in 
computer security.  The detection proceeds by finding correlated flows 
entering and leaving the network.  Traditional
approaches have used patterns inherent
in traffic flows, such as packet timings, sizes, and counts, to link
an incoming flow to an outgoing one~\cite{staniford-chen:oakland95,zhang:sec00,donoho:raid02,wang:esorics02,blum:raid04}.  More recently, an active
approach called \emph{watermarking} has been
considered~\cite{wang:ccs03,pyun:infocom07}.  In this approach,
traffic characteristics of an incoming flow are actively perturbed
as they traverse some router to create a distinct pattern, which can
later be recognized in outgoing flows.  These techniques also 
have relevance to anonymous communication, as linking two flows can 
be used to break anonymity, and both 
passive traffic
analysis~\cite{levine:fc04,danezis:pet04} and active
watermarking~\cite{wang:ccs05,wang:oakland07,yu:oakland07} have been
studied in that domain as well.

% FIXME: what about dropped or inserted packets

The choice between passive and active techniques for traffic analysis exhibits a tradeoff.  
Passive approaches require observing relatively long-lived network flows, and storing or 
transmitting large amounts of traffic characteristics.  Watermarking approaches are more efficient, 
with shorter observation periods necessary.  They are also \emph{blind}: rather than storing or 
communicating traffic patterns, all the necessary information is embedded in the flow itself. 
This, however, comes at a cost: to ensure robustness, the watermarks introduce large delays (hundreds of milliseconds) 
to the flows, interfering with the activity of benign users, and making them subject to 
attacks~\cite{peng:oakland06,kiyavash:sec08}.


Motivated by this, we propose a new category for network flow watermarks, the \textit{non-blind flow watermark}s. Non-blind watermarking lies in the middle of passive techniques and (blind) watermarking techniques:  similar to passive techniques (and unlike blind watermarks), 
non-blind watermarks will record traffic pattern of incoming flows and correlate them with outgoing flows.  
On the other side, similar to blind watermarks (and unlike passive techniques), non-blind watermarking aids traffic analysis by applying some modifications to the communication patterns of the intercepted flows. 
We develop and prototype the first non-blind flow watermark, called RAINBOW. 
RAINBOW records the \textit{timing} pattern of incoming flows and correlate them with the timing pattern of the outgoing flows. On each incoming flow,
RAINBOW also inserts a watermark by delaying some packets, after recording the received timings.  
As such a  watermark is generated independently of the 
flows, this will diminish the effect of natural similarities between two unrelated flows, and allow a flow 
linking decision to be made over a much shorter time period.  RAINBOW uses spread-spectrum techniques to 
make the delays much smaller than previous work.  RAINBOW uses delays that are on the order of only a few milliseconds; 
this means that RAINBOW watermarks not only do not interfere with traffic patterns of normal users, they are 
also virtually \emph{invisible}, since the delays are of the same magnitude as natural network jitter.
In \cite{houmansadr:ndss09} we use different information theoretical tools to verify the invisibility of  RAINBOW, and demonstrate its high performance in linking network flows through a prototype implementation over the PlanetLab~\cite{bavier:nsdi04} infrastructure. 

In this paper, we thoroughly analyze the detection performance of  RAINBOW non-blind watermark, and compare it with that of passive traffic analysis schemes. By using \textit{hypothesis testing} mechanisms from the detection and estimation theory \cite{poor88}, we find the optimum detection schemes for RAINBOW as well as the optimum passive detectors under different models for network traffic. Modeling  real-world network traffic  is a complicated problem as it depends on many different parameters; as a result,  we only consider two extreme models of the network traffic: (1) independent flows where each flow is modeled as a Poisson process (traffic model A), and, (2)  completely correlated flows where all flows are considered to have similar timing patterns (traffic model B). We assume that any real-world traffic model lies in the middle of these two extreme models. 
Our analysis leads to the following important conclusions: 

 i) Non-blind watermarking \emph{always} performs a better  detection than passive traffic analysis. This is an essential result in motivating the use of non-blind watermarks over passive traffic analysis, since both have similar scalability constraints, i.e., both approaches have $O(n)$ communication overheads and $O(n^2)$ computation overheads \cite{houmansadr:ndss09}. Not that this point is not necessary (nor is always true) to motivate the use of traditional (blind) watermarks over passive traffic analysis, since blind watermarks provide much better scalability (i.e., $O(1)$ communication overhead and $O(n)$ computation overhead \cite{houmansadr:ndss09} ).

 ii) Our analysis shows that the performance advantage of non-blind watermarking (over passive schemes) is only marginal  for uncorrelated network traffic, while it is very significant for correlated network traffic. This knowledge can be used to decide the best traffic analysis approach in various applications.
We validate our analysis through simulating the detection schemes on real network traces. In particular, we show that for highly correlated traffic, e.g., same webpage downloads, passive traffic analysis performs very poorly while a RAINBOW watermark is highly effective. 


 iii) We also show (through both analysis and experiments) that  the optimum watermark detector derived for correlated traffic (namely $SLCorr$) also performs very good for uncorrelated traffic (while the optimum watermark detector for uncorrelated traffic does not do well for correlated traffic). This allows one to use $SLCorr$ as the sole watermark detector regardless of the type of traffic being observed. This is especially useful in real-world applications where the observed traffic is a mixture of different flow types. 

Note that in this paper we do not discuss the performance advantage of non-blind watermarks over traditional blind watermarks, as this has been justified in \cite{houmansadr:ndss09}. 

%Our analysis in this paper shows that even though the optimum passive detector performs as good as  a watermark detector for uncorrelated traffic (traffic model A), however, it results in large false positive error rates in the case of correlated flows (model B). This is while  the optimum watermark detector performs well under both models of traffic. This \textit{justifies the use of non-blind watermarks over passive traffic analysis}, as a main conclusion of this research. 


%
%Motivated by this, we develop a new scheme for linking flows, called RAINBOW.  As with passive techniques, 
%our scheme will record traffic timings of incoming flows and correlate them with outgoing flows.  However, 
%we also insert a watermark value by delaying some packets.  As the watermark is generated independently of the 
%flows, this will diminish the effect of natural similarities between two unrelated flows, and allow a flow 
%linking decision to be made over a much shorter time period.  We use spread-spectrum techniques to 
%make our delays much smaller than previous work.  We use delays that are on the order of only a few milliseconds; 
%this means that our watermarks not only do not interfere with traffic patterns of normal users, they are 
%also virtually \emph{invisible}, since the delays are of the same magnitude as natural network jitter.

%We analyze our technique using a mathematical model of network traffic and delays.  We show that in our technique, 
%low-amplitude watermarks can achieve false-positive and false-negative rates that are an order of magnitude
%smaller than passive traffic analysis with short observation 
%periods---a few hundred packets. 
% We validate our analysis by building a prototype implementation of 
%our scheme.  We test it by generating flows with timings taken from real SSH~\cite{ssh:rfc4251} traffic traces,
% and linking flows that traversed the Internet between PlanetLab~\cite{bavier:nsdi04} nodes. 
%  Our scheme performed quite well in this setting as well.  Note that PlanetLab introduces significantly 
%more jitter than would be present in an enterprise network, so in practice, much lower watermark delays, or smaller 
%packet sizes, can be used. We also analyze the invisibility of our scheme by subjecting it to several 
%information-theoretic detection tools~\cite{gian:ccs07,peng:oakland06}. 

% FIXME: discuss how different jitter affects our watermark; e.g. in an Enterprise, jitter may be quite low

%We also extend our scheme to handle dropped or inserted packets.
%Such changes to flows will occur naturally due to packet losses,
%retransmissions, or repacketization.  By adjusting our scheme to
%perform \emph{selective correlation}, where packets that do not
%match up between the incoming and outgoing flows are dropped, our
%scheme can be made robust to packets being inserted
%and deleted, though at the cost of either longer observation periods
%or higher watermark amplitude.

The rest of this paper is organized as follows: we review the problem of stepping stone detection and existing schemes in Section~\ref{sec:background}.  Our RAINBOW  scheme is presented in Section~\ref{sec:NBSS}. In Section~\ref{sec:detection}, we use hypothesis testing to find and analyze the optimum likelihood ratio detectors for passive and non-blind active (watermark) approaches under different traffic models, and analyze their false error rates. In Section~\ref{sec:implementation}, we validate the analysis results through simulation of the detection schemes over real network traces. Finally, the paper is concluded in Section~\ref{sec:conclusionsFuturework}. 



%The rest of this paper is organized as follows: we review
%the problem of stepping stone detection and existing schemes
%in Section~\ref{sec:background}.  The RAINBOW
% scheme is presented in
%Section~\ref{sec:NBSS}. In Section~\ref{sec:analysis}, we use
%\textit{detection theory} to analyze performance of the proposed scheme.
%We provide implementation results in
%Section~\ref{sec:implementation}, validating the analysis. In
%Section~\ref{sec:selectivecorrelation} we extend RAINBOW by
%introducing \textit{selective correlation} to make it robust to
% flow modifications. Discussions on watermark invisibility
%are presented in Section~\ref{sec:invis}, and paper is
%concluded in Section~\ref{sec:conclusionsFuturework} along with
%some future research directions.
%TODO: address invisibilty tests
